The Untold Story of the Clones: Content-agnostic Factors that Impact YouTube Video Popularity

Video dissemination through sites such as YouTube can have widespread impacts on opinions, thoughts, and cultures. Not all videos will reach the same popularity and have the same impact. Popularity differences arise not only because of differences in video content, but also because of other "content-agnostic" factors. The latter factors are of considerable interest but it has been difficult to accurately study them. For example, videos uploaded by users with large social networks may tend to be more popular because they tend to have more interesting content, not because social network size has a substantial direct impact on popularity. In this paper, we develop and apply a methodology that is able to accurately assess, both qualitatively and quantitatively, the impacts of various content-agnostic factors on video popularity. When controlling for video content, we observe a strong linear "rich-get-richer" behavior, with the total number of previous views as the most important factor except for very young videos. The second most important factor is found to be video age. We analyze a number of phenomena that may contribute to rich-get-richer, including the first-mover advantage, and search bias towards popular videos. For young videos we find that factors other than the total number of previous views, such as uploader characteristics and number of keywords, become relatively more important. Our findings also confirm that inaccurate conclusions can be reached when not controlling for content.

==> oldergr.tex <==
\section{Empowering Rich-Gets-Richer}
\label{sec:ergr}

\subsection{First Mover Advantage}

Our evidence for the rich-gets-richer phenomenon suggests a
strong advantage to the video of a particular content that is \emph{first} made
available. The advantage of using the clone-based methodology over any other method here
is evident; we can  compare videos of identical content, and therefore
better evaluate the advantage of being the first to upload the content.

To track video popularity over time, we use YouTube's insight data collected through HTML
scraping. As a first step, we consider the success of the first mover in each cloneset, where
a success event for a particular video is defined as when that video accumulates the larger
number of total views compared to all other videos within the clone set.
We first consider how often the most succesful video within a clone set is the first to 
either be uploaded or discovered through search.
Table~\ref{tab:firstMover} shows the number of times the video clone that obtained the highest 
total view count was the first (or among the first four) videos in the clone set to be 
uploaded or found through search. Overall, the winner was uploaded first among
the videos in the clone set in 27.1\% of the observed cases, and was 
among the first five in 60.4\% of the cases. 
Similarly, the winner is the first to be found through search in 66.7\% of the cases 
for which we have (insight data) statistics, and among the first five to be found 
through search in 92\% of the cases. Clealy, there is a significant advantage to the first mover.

\begin{table}[th]
\centering
\begin{tabular}{|l|c|c|c|c|c|c|}
  \hline
 & 1st & 2nd & 3rd & 4th & 5th & later\\
\hline
%%Winner uploaded & 13  & 6    & 4   & 3   & 3   & 19\\
%%Winner searched & 8  & 1    & 0   & 1   & 1   & 1\\
Winner uploaded & 27.1  & 12.5    & 8.3   & 6.3   & 6.3   & 39.6\\
Winner searched & 66.7 & 8.3   & 0.0   & 8.3   & 8.3   & 8.3\\
 \hline
\end{tabular}
\caption{The percentage of times a video clone that obtained the highest total view count
was the first, second, third, fourth, fifth (or later) among the  videos in the clone set
with respect to being uploaded or searched.  (Clone sets with relevant statistics considered.)}
\label{tab:firstMover}
\end{table}


While the first mover is not always the winner,  the first mover is often 
 highly successful, even when it is not the winner.  To illustratre this, we consider
the view count of the first uploaded video relative to the winner.  A ratio 
of one corresponds to the case where the first mover is the winner, and 
a small  ratio indicates that the first mover was relatively unsuccessful.  
Figure~\ref{fig:ccdf-first-mover} shows the complementary cumulative distribution function (CCDF) 
of this ratio for our dataset.  In addition to the 27\% of clones sets where the first mover was the 
winner, this ratio is above 0.5 for 35\% and abobe 0.1 for 50\% of the first-movers.
Given the high skew in overall view counts, these values are high.
 
While these results suggest that the first mover typically is relatively successful 
it is interesting to note that there are cases where other videos have been able to 
surpass the first mover in popularity.  What is it that allow some other video overtake 
the spot as the most popular clone?  Section~\ref{sec:dynamics} takes a closer look 
at some influences that can cause such overtakings.

\begin{figure}[t]
\centering
\includegraphics[width=0.375\textwidth]{./graphs/fraction-of-views-ccdf.png}
\caption{The CCDF of the ratio of the view count of the first uploaded video in a clone set, 
relative to the view count of the video with the highest view count in the same set.}
\label{fig:ccdf-first-mover}
\end{figure}

\subsection{Video Discovery and Featuring}

Apart from the content-agnostic factors considered thus far, a number of 
system specific factors potentially impact views. Examples include featuring on YouTube, 
ranking of the video in YouTube search, and embedding of the videos on external sites. 
While these variables are difficult to capture over time, the `video referrers' part of the 
YouTube insight data provides (for some videos) additional information necessary
for this evaluation. The results presented here is based on analysis of clone sets
that have multiple videos with insight data. We use YouTube's classification of registered
referrers (cf. Appendix for a description of these referrers).

\begin{figure}[th]
\centering
\includegraphics[width=0.375\textwidth]{./graphs/referrers_fracviews_avgOFavg_cloneset_box_16categories_top2.png}
%%referrers_time_box_16categories_top2.png
\caption{Boxplot of the average fraction of views (per cloneset) coming through different referrer categories.}
\label{fig:boxplot-fracviews-cloneset}
\end{figure}

In this section we take a closer look at the impact system specific factors may have on the success of a video.  
In particular we compare how the most successful videos within each clone set obtain their views, relative to 
how their less successful counterparts  obtain views.
 
%%{\bf Anirban - need to be careful here. A video X may become popular because of 
%%external searches and so on. Alternatively, we may see more searches for the 
%%popular content simply because the content is popular.}
Figure~\ref{fig:boxplot-fracviews-cloneset}  compares the average fraction of views 
coming through different referrer types for the most popular clones, with that of 
the remaining clones.\footnote{We present the mobile referrers separately
as an access that is done with a mobile device may be Google
search links, external links, or embeds, for example.
It is, however, an intersting measure as the use of a mobile device
may reflect a more social-based engagement.}
The results are somewhat counter-intuitive. Notice that 
the most popular videos are not necessarily the videos that are 
prominently featured or externally linked.  Instead, the search and mobile referrers 
account for most of the difference. For example, for the both the mobile and the YouTube search referrer category, 
the median of the top clones is almost equal to the 90th quartile of the remaining videos.
On the other hand, the less successful clones get most of their views through related (video) referrals.


%%\textcolor{red}{NOT CLEAR. Note that mobile referrers may be Google 
%%search links, external links, or embeds for example, but could not be identified
%%by Youtube because the majority of newer mobile browsers support
%%opening a new window or tab when clicking on a video outside Youtube, in which case 
%%the the referrer is lost. And thus a clear classification
%%of the mobile sources cannot be obtained, but one could say that in general,
%%mobile devices reflect a more social-based engagement.}

%For the less popular clone, a high fraction of views is coming through related videos
%referrers. (Probably need to check that most of the related referrers come from the top clones? 
%It would be good to have it as a statement).

\begin{figure}[!t]
\centering
%%\begin{tabular}{cc}
%%\includegraphics[width=0.375\textwidth]{./graphs/fb-google-count-external.png} &
\includegraphics[width=0.375\textwidth]{./graphs/fb-google-views-external.png}\\
%%(a) Featured & (b) Externally Linked\\
%%\end{tabular}
\vspace{-10pt}
\caption{The fraction of views coming through external sources, for clones that are externally linked.}
\label{fig:bar-fracviews-extra}
\end{figure}

Figure~\ref{fig:bar-fracviews-extra} shows the fraction of views coming through external
referrers only (not including embeds). Note that Google is shown as an external
source of traffic and it is  driving most of the external views of the
popular clones.  Google is considered an external referrer because 
views may come from a number of Google non-search services such as 
Google News, Google Reader, and Google Group posts.

Overall, the highest fraction of clicks to a video is coming through the search referrers.
As all videos can potentially be found through search, but not all videos are featured 
or embedded on external websites, we take a closer look at these referrers. 
Figures~\ref{fig:boxplot-fracviews-clone-extra}(a) and~\ref{fig:boxplot-fracviews-clone-extra}(b)
show the corresponding boxplots of the fraction of views coming through different referrer types
for only the clones that are featured and externally linked, respectively.
The same conclusion applies to these data subsets: search referrers are the most
powerful in terms of the percentage of traffic they bring, whereas 
 search and mobile referrers are still showing the biggest differences between successful
and less successful videos. 

Recall that we are considering multiple copies of the same content, and this
allows us to remove biases introduced because of differences in content (e.g., a popular
content is more likely to be searched than a non-popular one).  
Our results suggest that successful videos are much more 
prominently selected through searches.  This could potentially occur because of 
YouTube's internal search mechanism, the keywords associated with the video, the
keywords entered by the users, or a combination thereof.  
\textcolor{red}{
Such biases may further skew the bias in the case people pick the first search 
results, rather than from lower down on the list.  The popular videos may also 
benefit from people preferring content that have higher view counts 
(visible to the user)~\cite{SaWa08}.}


%Again, we note that our unique dataset allow 
%us to remove the importance of content.  This is an important observation as we can eliminate 
%the obvious bias that some videos have more views because more people searched for that content.  
%Instead, videos with a higher fraction of views due to searches (within a clone set) must either 
%have been more frequently returned by the search engine or more frequently selected by the user, 
%than the other clones. 

%%\textcolor{red}{AM: NEED to flush this out.
%%It is likely that the most popular clones are more prominent in searches,
%%and thus a video gets an unfair percentage
%%of views due to search just because it is in the top ranking list.}

\textcolor{red}{
Next, we statistically test whether or not the search is providing additional bias towards more popular clones,
and enabling the videos with larger view counts to attract even more views. 
For each clone set, we compute the fraction of views coming from search for the top ranking clones ($x_i$),
and  the fraction of the total views accounted by top ranking clones ($y_i$).
Each ($x_i$,$y_i$) pair is an observation.
If there is no additional (unproportional) bias in the search methods,
the ratio $x_i / y_i$ should be bigger than 1 only half of the time.
Figure~\ref{fig:slopetest} shows a scatter plot of this ratio against 
the median age of the videos in each clones set when considering the top 2 two clones
in each set.  We note that 10 of the points are above the $x/y=1$ line and only 5 are below the line.
The probability for this observation in the case there was no bias is 0.171.
This suggest that there is a search bias.  
The figure also suggests that the bias is caused by the younger clone sets.}

\begin{figure}[!t]
\begin{center}
\includegraphics[width=0.375\textwidth]{./graphs/referrers_searchbias_median_age_top2.png}
\caption{Search bias towards top 2 videos in each clone set versus the median age of the videos in each clones set.}
\label{fig:slopetest}
\end{center}
\end{figure}

\textcolor{red}{
More formally, we can use hypothesis testing to systematically quantify the
likelihood that the search mechanism is proportionally fair given the observed results.
Similar to the scale-free rich-gets-richer models,
proportional fairness would ensure that views from search is proportional to the total view count.
We formulate the null hypothesis, denoted $H_0$, as the ``search mechanism is fair''.
Mathematically, we express the null and alternative hypothesis as:
\[{H_0}: P(x_i>y_i) = 0.5\]
\[{H_a}: P(x_i>y_i) \neq 0.5\]
where $p = P(x_i>y_i)$ is the probability of observations below the $x/y = 1$ line.
We estimate the standard deviation and calculate the
the test statistic $z$, which measures how far the sample mean $p$
diverges from the expected mean of a fair search mechanism.
We then compute the p-value of the test statistic and conclude
whether or not the null hypothesis is rejected.
We choose a 95\% confidence interval, and so the level at which
we reject the null hypothesis is 0.05. Table~\ref{table:hypothesis-fair}
shows the p-values for a different subsets of the most popular clones (top 1,
top 2, top 3, and top 4 ranking videos). 
While the null hypothesis only is rejected for the top 3 case,
we note that we get relatively small p-values for the other cases as well. 
We believe that a larger dataset would help further validate our observations.} 

We surmise that YouTube's search mechanism, at the time of
these measurements, either was biased towards the most popular clones 
or in the case multiple clones are presented to the user, the users are biased towards picking 
the videos with higher view counts.
This naturally, empowers the rich-gets-richer phenomenon.
In summary, among the documented referrers, the search referrers
is an important factor that has significant impact on a clone's
popularity.

\begin{table}[th]
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\hline
 & Top 1 & Top 2 & Top 3 & Top 4\\
\hline
p-value & 0.075 &  0.171 & 0.035 & 0.285 \\
\hline
\end{tabular}
\caption{Hypothesis testing of whether or not the search mechanism is unproportionally 
biased towards the most popular clones.}
\label{table:hypothesis-fair}
\end{center}
\end{table}


\begin{figure*}[!t]
\begin{center}
%%\begin{tabular}{cc}
%%\includegraphics[width=0.45\textwidth]{./graphs/referrers_fracviews_avgOFavg_clone_externalaggregate_top2.png}&
%%\includegraphics[width=0.45\textwidth]{./graphs/referrers_fracviews_avgOFavg_clone_featuredaggregate_top2.png}\\
\begin{tabular}{cc}
\includegraphics[width=0.375\textwidth]{./graphs/referrers_fracviews_external_box_13cat.png}&
\includegraphics[width=0.375\textwidth]{./graphs/referrers_fracviews_featured_box_13cat}\\
(a) Externally linked clones &
(b) Featured clones\\
\end{tabular}
\caption{Boxplot of the fraction of views of clones externally linked and featured, 
coming through different referrer categories.}
\label{fig:boxplot-fracviews-clone-extra}
%%\label{fig:boxplot-fracviews-clone-external}
\end{center}
\end{figure*}

%how certain you are of the result of a statistical experiment.
%How can we tell if the search meachanism is fair?
%http://20bits.com/articles/hypothesis-testing-the-basics/


As previously discussed in this section, first mover advantage can be important 
for the success of a video.
In addition to being uploaded, it is important that the video is discovered 
and/or made available through different paths.  Using correlation analysis, 
we have observed that there often is a significant positive correlation 
between the total view count and the order in which clones are first referrered, 
featured, or accessed through mobile devices.  While omitted, these results suggest 
that there is also is a \textit{first-discovery advantage}, where videos discovered 
earlier through internal search methods, featured earlier, or that is accessed through 
mobiles earlier, tend to be ranked higher.




%%
%%% latex table generated in R 2.11.1 by xtable 1.5-6 package
%%% Mon Sep 12 20:51:56 2011
%%\begin{table}[th]
%%\begin{center}
%%{\tiny
%%\begin{tabular}{|c|l|l|l|l|l|l|}
%%  \hline
%% & External & Featured & Internal & Search & Mobile & Social \\
%%  \hline
%%17 & -0.179 & 0.625 & 0.166 & 0.269 & 0.455 & 0.000 \\
%%  22 & 0.281 &  & 0.065 & 0.271 & 0.597 & 0.000 \\
%%25 & 0.865 & 1.000 & 0.602 & 0.765 & 1.000 & 1.000 \\
%%  37 & 0.520 & 1.000 & 1.000 & 0.876 & 0.988 & 0.000 \\
%%38 & 0.375 & 1.000 & 0.724 & 0.591 & 0.803 & 0.000 \\
%%  42 & 0.268 & 0.500 & 0.526 & 0.686 & 0.111 & -1.000 \\
%%43 & -0.093 & 1.000 & -0.330 & 0.683 & 0.528 &  \\
%%  45 & 0.807 & 0.869 & 0.520 & 0.781 & 0.893 & 0.000 \\
%%46 & 0.370 & 1.000 & -0.046 & 0.653 & 0.852 & 0.000 \\
%%  49 & 0.333 &  & 0.354 & 0.955 & 0.613 & 0.000 \\
%%50 & 0.566 &  & 0.390 & 0.695 & 0.740 &  \\
%%  51 & 0.220 & 0.720 & 0.588 & 0.470 & 0.657 &  \\
%%    \hline
%%\end{tabular}
%%}
%%\caption{{\bf CUT (for discussion, see extended version from email)} 
%%Pearson correlation between the ranks and observation order}
%%\label{table:corr}
%%\end{center}
%%\end{table}

%%\begin{figure}[!t]
%%\begin{center}
%%\includegraphics[width=0.45\textwidth]{./graphs/referrers_fracviews_external_count.png}
%%\caption{The fraction of links of externally linked clones, coming through external sources.}
%%\label{fig:pie-fracviews-external}
%%\end{center}
%%\end{figure}


==> oldintr.tex <==
\section{Introduction}

Videos on services such as YouTube can have widespread
impacts on opinions, thoughts, and cultures. Of course, not all videos become
equally popular and have the same  impact. What factors cause some videos to 
become more popular than others? In this paper, we provide a qualitative and 
quantitative answer to this fundamental question. 

Several factors impact the popularity of user-generated videos. 
The quality of the content, for example whether or not the video is  ``interesting'',
 is one key factor.  In addition, there are many ``content-agnostic''
factors  such as the video uploader's social network size, the video's current
view count, the video's title, the keywords associated with the video, and 
the service provider's search and featuring algorithms that  also influence 
a video's popularity. Since both content-related and content-agnostic factors
impact video popularity, understanding how content-agnostic factors influence
 popularity, and separating the influence of content and non-content related
factors has been challenging. For instance, videos uploaded by users with large 
social networks may tend to become more popular  because they generally upload
more interesting content, not because social network size has any direct impact 
on popularity. 
 

%YouTube is the world's largest video sharing community.  Today, the six-year-old 
%Website hosts millions of user-generated video clips, with roughly 48 hours of content 
%uploaded every minute, and three billion views per day~\cite{youtubeBLOG}.  
%While the most popular videos have the power to impact opinions, thoughts, and culture, 
%not all content will reach the same popularity and have the same impact.

%%Underlying this discussion, there is a fundamental question: 
%%What is it that makes some videos more popular than others?

%Popularity evolution is a complex process dependent on several endogenous and 
%exogenous factors~\cite{CrSo:08, Salganik:06}.  
%%%Culture, social psychology, personal psychology, perception, 
%%%belief, and even luck may shape how the content popularity 
%%%evolves~\cite{CrSo:08, Salganik:06}.  
%Understanding the popularity growth patterns of user-generated video content 
%is valuable for several reasons. Online popularity impacts the profits of 
%entertainment business, marketing and advertising industries.  
%In fact, the survival of many commercial products, media, recreation and technologies 
%rely on a significant user base. Understanding online popularity may therefore help 
%us build a better understanding of the underlying social and collective human 
%dynamics~\cite{CrSo:08}, as well as design better caching and content distribution 
%approaches~\cite{Moon:07, Applegate:2010}.

The increasing  interest in user-generated videos has spawned 
much work on  characterizing, modeling, and predicting video  popularity.
 User-generated video accesses at campus networks have been
characterized~\cite{Mahanti:07, Zink08}. Both static and
temporal properties of view counts to a collection of user-generated 
videos have been studied~\cite{Cheng:07, Moon:09, MAY+09, Borghol:11}. 
Models have also been proposed for video popularity evolution~\cite{Huberman:10, Moon:09, Borghol:11}. 
Many of these models are variations of  the classicial  {\em rich-get-richer} phenomenon~\cite{Barabasi:99}, 
which suggests that a video's current popularity as measured by its current total view count,
 is an indication of its future popularity~\cite{Huberman:10, Moon:09}.  
However, prior studies used datasets that consist of completely different content, 
and thus could not provide an unbiased model or insight about the underlying 
dynamics driving the popularity process. Instead, part of the difference in 
the observed popularity is simply because some content is better than others
 and naturally attracts more views. 

In this paper, we develop and apply a methodology that is able to accurately assess
the impact various content-agnostic factors have on  popularity. Our methodology is based on
studying the dynamics of identical copies of a video content. We refer to videos with the same content as {\em clones}. 
 This approach allows us to control bias introduced when studying videos that
do not have the same content. By collecting and analyzing clones from a 
range of different video contents, we are able to study the
impact video content has on popularity. In a nutshell, 
the key  contributions of this work are as follows:
\begin{itemize}
\item We develop a clone-based methodology for studying factors 
impacting video popularity. We show that one gets inaccurate results when 
not controlling for video content (i.e., when not using a clone-based methodology).  
\item When controlling for video content, we observe linear rich-gets-richer, 
with view count being the most important factor excepting for very young videos.
\item When controlling for video content, for young videos we find a variety 
of other significant factors, including uploader characteristics such as size 
of social network, and number of keywords.
\end{itemize}
An overview of our contributions is presented below.

%%Our first contribution is the dataset. 
Through extensive exploration, search, and viewing of YouTube videos, 
we identified 50 different video contents, each of which contained 
between 20 and 104 video clones. We call a group of identical videos
a {\em clone set}. In total, we identified 1, 908 clones. 
For each video, we used the YouTube developer's API  and HTML scraping to extract 
video information and statistics. 
%%{\bf AM: Are we using all snapshots? If not the following 
%%sentence needs to change.} We tracked the statistics to these videos over a three week period.
Using two snapshots, separated by a week, we collected both lifetime statistics 
and rate-of-change statistics for these videos. 
By analyzing the relative difference in popularity dynamics within clone sets, 
the individual heterogeneity bias, introduced by differences in content, 
is controlled and we can provide an unbiased analysis. We believe this 
dataset is unique, and plan to release it to the research community for 
further analysis. 
%%This allow us to 
%%better understand what factors allow a video, with the exact same content 
%%as some set of other videos, to attract more views. This novel dataset 
%%allows us to answer questions that could not be answered in previous studies.

%%Our second contribution is a detailed study
We apply multivariate linear regression and other statistical methods  to systematically
determine the factors that most influence a video's future popularity.
In particular, by analyzing a large number of explicit measurable factors which are provided
through the YouTube API, we find that the most significant 
content-agnostic  factors are the total view count, the video age,
 and the uploader's social network. We also show that determining the relative importance of
these content-agnostic factors  without controlling for video content would
result in the conclusion these factors are relatively
more important (compared to view count) than they really are.

Our dataset and analysis approach allows us to assess how
video content impacts popularity. In particular, we present a
detailed statistical analysis of the rich-get-richer model, and present
several important findings. We provide quantitative evidence for the existence of 
rich-gets-richer phenomena when differences owing to  content is eliminated. Using regression 
analysis and statistical hypothesis testing we show that video popularity follows 
a scale-free rich-gets-richer model with power-law exponent equal to one when 
the content of the individual videos is accounted for. However,
if the clone identity is not taken into account, the preferential selection 
of more popular videos is weaker, not scale-free, and with a power-law 
exponent smaller than one.  

While the total view count is the strongest predictor, other 
non-redundant factors can help explain various other aspects of the 
popularity dynamics. For example, the uploader's social network can 
be a good predictor for newly uploaded videos, and the video 
age can help differentiate videos at similar view counts that are 
accumulating views at different rates. We also find that similar 
analysis that does not account for content, would considerably
underestimate the impact of various non viewcount
factors (e.g., number of keywords) when considering recently-uploaded videos.

Leveraging our dataset we are also able to provide concrete 
evidence of the first-mover advantage (i.e., the favorable impact of being the first to upload
a video).  We also take a closer look at  other external influences that in some cases may 
outweigh the first-mover advantage, including a strong uploader network or extensive featuring of the
video in blogs and other sites.  
Finally, we take a closer look at distinguishing features of the most 
successful clones.  We find that the most successful clones are accessed 
through search unproportionally often (relative to the search accesses of 
less popular clones), which can significantly boost their popularity and 
in some cases also eliminate the first-mover advantage.

{\bf AM: need to update this.}
The rest of this paper is organized as follows.
Section~\ref{sec:related} discusses related work.
Section~\ref{sec:methodology} describes our clone-based methodology,
our datasets, and the analysis approach made possible by our unique dataset.
Section~\ref{sec:ImportantFactors} discusses the measurable variables used for 
the analysis and examines their impact on future video popularity.
%%including a detailed study of the rich-gets-richer phenomenon.
%%Section~\ref{sec:identity} analyze the impact of content and video identity,
%%and include a detailed study of the rich-gets-richer phenomenon.
%%first-mover advantage phenomena.
%%Section~\ref{sec:rgr} provide a detailed study of preferential attachment and the 
%%first-mover advantage phenomena.
Section~\ref{sec:dynamics} presents 
an analysis of popularity dynamics,
including a detailed study of the rich-gets-richer phenomenon, and 
an analysis of some other external influences on the video popularity, 
including a closer look at the first-mover advantage and the impact different 
factors have on very young videos. 
Section~\ref{sec:conclusions} concludes the paper and gives directions for future work.  


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% COMMENT OUT REST OF SECTION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\comment{
\section{Introduction}

%% What is the specific problem considered
YouTube is the world's largest video sharing community.  
With 48 hours of user-generated content uploaded every minute, 
and 3 billion views a day~\cite{youtubeBLOG}, the six-year-old website has
grown to become the most visited online video-sharing site.
With millions of user-generated clips on YouTube, 
what is it that makes some videos more popular than others?

%% Motivation
Popularity evolution is a complex 
process dependent on several endogenous and exogenous factors.
Culture, social psychology, personal psychology, perception, belief, and even luck shape 
how the popularity of content evolves~\cite{CrSo:08, Salganik:06}. 
Understanding the popularity growth patterns of user-generated video content is 
valuable for several reasons. Online popularity impacts the profits of entertainment business, marketing and advertising industries, simply because commercial products, media, recreation and technology survives on grounding popular content. Online popularity has the power to impact the dynamics of opinions, thoughts, and culture. Understanding online popularity is important to comprehend the underlying social and collective human dynamics~\cite{CrSo:08}, and is crucial to tackle system design issues like caching and content distribution approaches~\cite{Moon:07, Applegate:2010}.

%% Motivation w/r to related work
There has been growing interest in analyzing the popularity characteristics and prediction of 
the user-generated video content on YouTube. 
Previous studies have focused on a static snapshot of video view counts, or on the evolution
of view counts, and several models have been proposed for predicting the popularity growth rates 
of videos. Most of the previous models suggested a {\em rich get richer} phenomenon, where the current 
popularity of a video is an indication of its future popularity. 
These studies however are examining the similarities of videos that are completely different,
and thus fail to capture an unbiased model of the underlying system driving the popularity process.
Some content is simply better than other content and naturally attracts more views.  

In this paper, we study and model how viewing rates of user-generated videos with
the exact same content, which we refer to as {\em clones}, 
change over time. We make several contributions that address the identified problem.

Our first contribution relates to the novel data collection methodology.
In this work, we collected a dataset of video clones and used 
the YouTube developer's API~\cite{youtubeAPI} to extract their information, statistics
and insight data. We tracked the views to these videos over a three week period.
By looking at clones, the individual heterogeneity bias, introduced by the difference in
content, is controlled. And thus, an unbiased analysis could be conducted to understand
what factors allow a video, with the exact same content as other videos, to attract more views. 
This interesting dataset allows us to answer questions that could not be answered in previous studies. 
%The clones dataset addresses the bias issue introduced in the 
%analysis of user-generated video popularity of distinct content.


Our second contribution is a detailed investigation to identify the important factors
that impact a clone's popularity. We performed a multivariate linear regression,
a collinearity analysis and a principle component analysis on the individual clones of the dataset,
their aggregate and their aggregate when clones identity is taken into consideration (dummy variables). 
The key findings show that there are multiple variables that strongly influence
the popularity dynamics of user-generated video clones, but many of the identified
variables are redundant. The most significant non-redundant factors are
the total viewcount and the quality of a video, and the social network of its uploader.

Our third contribution is an age-based regression analysis that examines
the evolution of important factors in time. First, we show that the total viewcount
of a video is the strongest predictor of its popularity after a certain age threshold.
Second, we show that in the early stages of a video lifetime, the uploader social network 
becomes a factor as important as the total viewcount, in affecting a clone's popularity. 
We also show that the number of video keywords, a factor that has no impact
in later stages of a video lifetime, is more significant than the total viewcount in the beginning.
When videos are younger than 3 days, we can see that approximately 62\% of the variation in views 
can be explained by the keywords number alone. The number of keywords is 
the major factor behind the discovery of videos through search mechanisms.

Our forth contribution is examining the external factors' impact on the popularity
of user-generated clones. We demonstrate that although the most popular clones
within a cloneset are slightly more featured, the highest fraction of views to
these videos occur through the "video search" method. (Only?? More analysis needed here)

Our fifth contribution is providing quantitative evidence for the existence of 
preferential attachment when the initial attractiveness (due to difference in
content), is eliminated. Using regression analysis and statistical hypothesis tests, 
we show that for the individual clonesets, and the dummy variables model,
the popularity evolution is scale free, and strongly controlled by rich-get-richer behavior.
For the aggregate model, we observe an exponential popularity evolution
that could be more biased towards random selection instead of rich-get-richer dynamics.
We also investigate the video age effect on preferential attachment and 
prove the presence of first-mover advantage. The examination of the 
first-mover advantage was possible due to 
our unique dataset that allows us to restrict the set of videos analyzed to those that are exactly similar. 
%testing for the existence of a preferential
%attachment process. We examine the rate increase in views versus the 
%current viewcount distribution using univariate linear regression on the log-log scale.

(Our sixth contribution, prediction??)

%Outline
The rest of this paper is organized as follows.
Section~\ref{sec:data}
describes our data collection methodology.
Section~\ref{sec:related} discusses
related work.
Section~\ref{sec:ImportantFactors} discusses all the variables
used for analysis and examines the factors that impact the popularity of videos.
Section~\ref{sec:AgeAnalysis} presents an age based analysis
of the significant factors. Section~\ref{sec:rgr} discusses the 
the existence of preferential attachment and first-mover advantage phenomena.
Section~\ref{sec:conclusions} concludes the paper and gives directions for future work.
}




==> oldrgr.tex <==
\section{Rich-gets-Richer Models}
\label{sec:rgr}

Prior works have suggested that the future popularity follows a rich-gets-richer 
phenomenon~\cite{Barabasi:99} or a variant thereof (e.g.,~\cite{Huberman:10, Moon:09}), 
which suggested that the viewing rate of a videos is proportional to the current  total views 
to the video. More specifically, it has been suggested that the probability $\Pi(v_i)$
that a video $i$ with $v_i$ views will be selected for viewing
%%to acquire a new view depends on the viewcount $k_i$ of
%%video i, such that:
%%\[ \Pi(k_i) = \frac{k_i}{\sum{k_j}} \]
%%where the rate increase
follows a power law
\[ \Pi(v_i) \propto v^{\alpha}, \]
where $\alpha$ is the power exponent.

Perhaps, the most interesting case is when $\alpha=1$, which was 
considered by Barabasi and Albert~\cite{Barabasi:99}; this corresponds to 
linear preferential attachment, and can be shown to result in a scale-free distribution.
For the more general non-linear case, the underlying distribution depends strongly on
the parameter $\alpha$ and the scale-free characteristics no longer holds~\cite{Krapivsky2000}.
In the sub-linear case ($\alpha<1$) the rate increase follows a stretched exponential
distribution. In the super-linear case ($\alpha>1$), the rich gets much richer, and
when $\alpha>2$ a winner-takes-all phenomenon quickly occurs.

% SA: nice analogy but IMO the above explains itself. if we have space?
%{\bf AM - As mentioned by Sebastien, this discussion can be cut.} 
%We note that these
%cases can be compared against a bank giving differentiated interest rates on their
%customers savings.  The linear case simply corresponds to the case where everybody
%gets the same interest, but whoever has more money naturally will gain more money
%than those with less money.  Similarly, the sub-linear case corresponds to the case
%where people with less money will be given a higher interest rate, such as to help
%them catch up with the richer people, and of course, as suggested by the winner-takes-all
%phenomenon, for example, the super-linear case have opposite effect.

Notice that  rich-gets-richer models do not take 
into account any  factor other than the total view count. Our analysis, however, has shown 
that (i) when controlling for video content, several content-agnostic factors 
appear to have high predictive power, with the current total view count and the 
video age being the most important factors, and (ii) the content itself is a 
significant contributor to the video's popularity. A natural follow-up question is the
following: Do rich-get-richer models apply in the restrictive case where 
there are multiple {\em active} videos that are similarly aged? 

\begin{table*}[!t]
\begin{center}
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{} & \multicolumn{1}{|c|}{Slope estimate} &
\multicolumn{2}{|c|}{Confidence intervals} & \multicolumn{3}{|c|}{Hypothesis testing}\\
\hline
Metric        & $\alpha~(\sigma)$ & 90\% & 95\% & H0: $\alpha = 1$ & H0:$\alpha \ge 1$ & H0:$\alpha \le 1$\\
\hline
Individual    &  1.027 (0.091) & 0.988-1.065 & 0.981-1.073 & 0.85 & 0.57 & 0.43 \\
%%\hline
%%Median        &  1.066 (0.09)& - & -  &  0.307 & 0.73 & 0.27\\
\hline
Content-based &  1.003 (0.014) & 0.98-1.027 & 0.976-1.031 & 0.81 & 0.59 & 0.40 \\
\hline
Aggregate  &  0.932 (0.016) & 0.906-0.958 & 0.901-0.963 & REJECTED & REJECTED & 1.00  \\
\hline
\end{tabular}
\caption{Rich-gets-richer slope estimates and hypothesis testing.}
\label{table:slope-hyp}
\end{center}
\end{table*}

\textcolor{red}{
We proceed as follows with our analysis. For each clone set, we first find the video clone 
that has seen the most increase in views within our measurement window of one week.  This 
video is considered the most active clone.  Our analysis then only considers the videos in 
the clone set that were uploaded within two years of the upload time of the most active clone.  This more 
restricted age-window reduces the age factor while still keeping most videos within clone sets.}

%%We proceed as follows with our analysis. For each clone set, we find the video clone
%%that has seen the most increase in views within our measurement window of one week.
%%Effectively, we determine which video clone had the highest viewing rate within 
%%the measurement window. We then look for other videos in the clone set that
%%are within two years of the upload of the clone with the largest view count increase.
%%The two year window on both sides of the most active clone, although somewhat 
%%arbitary, allows us to consider a large number of clones while reducing the impact
%%of the video age on our analysis. 

We now take a closer look at the impact differences in video identity
can have on the rich-gets-richer phenomena.  We examine how the rate at which videos attain new
views depends on the total view count using univariate linear regression (using log-transformed data).
All three analysis approaches, namely regression analysis on individual clone sets, on the aggregate, and 
the aggregate considering content identity, were applied. Using hypothesis testing, 
we determine if the system is sub-linear, linear, or super-linear.
Table~\ref{table:slope-hyp} summarize our results.

The first column in Table~\ref{table:slope-hyp} shows the coefficient estimates and standard
deviation resulting from the univariate regression analysis.
The second and third columns show the corresponding confidence intervals.
The results indicate that the slope estimates often are around one and
that the rate at which videos acquire views is correlated
with their current total view count, providing quantitative evidence for the existence of preferential
attachment. For the individual clone sets, and the extended content-based model, $\alpha$ is typically
equal or slightly higher than one.  The attachment rate is linearly dependent on the current total view count,
proposing that the popularity evolution is scale free,
and strongly controlled by rich-get-richer behavior.
For the aggregate model, $\alpha$ is less than one, indicating an exponential popularity evolution
that could result in a much even popularity distribution that suggested by the pure (linear)
rich-get-richer dynamics.

To validate these observations, we performed hypothesis testing
to check whether each slope estimate is linear, super-linear, or sub-linear.
Columns 4 through 6 in Table~\ref{table:slope-hyp} show the p-values of  the hypothesis tests.
%%We then perform hypothesis testing
%%to check whether this estimate is sufficiently equal to one, and not by random chance.
%%We actually perform three hypothesis tests.
These columns present results for  the hypothesis
that $\alpha$ is equal to 1 (linear preferential attachment), 
the hypothesis that $\alpha$ is greater than 1 (super-linear),
and the  hypothesis that $\alpha$ is less than 1, respectively.
Here, the p-values express the results of the hypothesis test as a significance level.
If p-values are smaller than 0.05, the hypothesis is rejected.
Using standard hypothesis testing,
we remind the reader that these tests can only answer if the hypothesis can be rejected;
not if the null-hypothesis is true.  However,  note that if two out of three (mutually 
exclusive) hypothesis are rejected,
this would suggests that the third hypothesis likely is true.

We note that the hypothesis testing in fact validate many of the observations based on our
discussion of the slope estimates.  In particular, it is clear that a model that does not
take the clone set identity into account (e.g., the aggregate model) 
may suggest a much weaker sub-linear relationship
than if the clone identity is taken into consideration.  Note that we can reject both the
hypothesis that the aggregate is linear and that it is super-linear.  This clearly suggest
that it is in fact  sub-linear.  Further, the extended model that takes into account
the clone set identity does not allow us to reject any hypothesis, but the values suggest that
linear relationship is pausible.
%%In the dataset we're analyzing, there is no individual heterogeneity
%%in terms of content among clones, so what makes a difference?
The results are interesting as they provide evidence for linear
(and in some cases even super-linear)
preferential attachment once we control the individual heterogeneity in content.




==> related.surveystyle.tex <==
\section{Related Work - Survey?}
\label{sec:related2}

\subsection{Static popularity characteristics}

Both Gill et al.~\cite{Mahanti:07} and Zink et al.~\cite{Zink08} 
relied on network traffic traces from a network gateway. 
They analyzed YouTube video requests from a campus network
and observed that the video requests follow a Zipf-like distribution
and  substantial network bandwidth savings would be feasible
if large proxy caches were used. Zink et al.~\cite{Zink08} performed 
a trace-driven study of caching policies confirming the
benefits of local edge network caching. 

Other studies on static popularity characteristics were based on meta-data sampled 
from video sharing services~\cite{Moon:09, MAY+09}. 
Cha et al.~\cite{Moon:09} analyzed the consumption pattern and popularity distribution of YouTube videos
and found that the total views since upload for videos of various ages is best fit 
by a power law distribution with exponential cutoff, and thus popularity is explained by a rich-get-richer model.
The exponential decay observed in the tail of the total views distribution
was explained using a "limited fetch" model, 
where some users do not request the same content many times,
and by information filtering by recommendation and search engines, 
where only a small number of popular items is returned.
To our knowledge, ~\cite{Moon:09} is the first work that studies the existence of "aliases"
(identical copies for a single UGC content), and its impact on the system characteristics.
Cha et al. definition of an alias is more flexible than our definition of a clone, 
as they consider a video having non-overlapping parts up to 1min as an alias. 
Simple analysis was conducted to demonstrate that content aliasing reduces 
the significance of a content popularity.
Cha et al.~\cite{Moon:09} were also the first to show 
a strong correlation between viewcount and the user participation, 
but they limited the user participation to one popularity metric,
the number of ratings. They reported the absence of any correlation between the video viewcount and its upload time, which 
is confirmed in our results. However, their analysis doesn't go deeper than pairwise correlation 
to evaluate the impact of the video age on its popularity. 

\cite{MAY+09} compared four popular video sharing workloads and established the presence of "invariants" among their characteristics. One of their main identified invariants is the heavy-tailed lifetime popularity of videos across the four sites, without specifying a particular model as a better fit for the data.

%Similar observations apply to other video-sharing services, based on data collected
%by sampling videos from these services~\cite{MAY+09}.
%Using multiple snapshots of meta-data from Dailymotion, 
%another popular video-sharing service, Mitra et al.~\cite{MAY+09}
%studied the effectiveness of total views popularity in 
%making caching decisions and found them to be 
%ineffective for large caches owing to changes in 
%the viewing rates of videos. 

% => check related work of first step, about cheng

More recently, Zhou et al.~\cite{Zhou:10}
studied the influence of some of YouTube's referrers
on views to videos: the featured, search and related videos
referrers. They observed that Youtube search and the related videos 
recommendation system are the most important source
of traffic to videos. Analysis was based on two datasets, 
one consisting of video requests at a university network gateway, 
and the other consisting from an initial set of featured videos,
and their related videos, collected recursively for three levels.  
They also observed a strong correlation between 
the views to a video and the number of views of its 
related videos, and suggest to consider it as a factor
in video popularity prediction.

Cheng et al ~\cite{Cheng:07} studied the relationship of related videos on YouTube
and showed that the related video graph has small-world characteristics
and has a large clustering coefficient.



\subsection{Popularity dynamics}

Studies have focused on the temporal aspects of the popularity dynamics. 

\subsubsection{Characterization}

Figueiredo et al.~\cite{Figueiredo:11} study the
popularity dynamics of three different YouTube video datasets; the 
three datasets considered are a sample from the most popular video lists,
a list of deleted videos, and a sample of videos obtained via keyword searches.
Similar to us, Figueiredo et al. utilize the recently available 
feature of the YouTube API that provides high-level statistics, 
the "Insight Data". For each video, they collect the popularity growth
curves and the referrers listed by Youtube. 
Figueiredo et al. show that the popularity characteristics of the three datasets
are different, and that among
different types of referrers, search and internal mechanisms
are the most important sources of traffic to Youtube videos.
Figueiredo et al. 
studied the significance and effect of external factors on the 
popularity evolution of videos, but their analysis was limited to 
the video referrers. 

Authors in ~\cite{Chatzopoulou:10} studied the popularity evolution of a collection of videos, instead of individual videos,
by grouping videos into age bins. Starting from the standard feeds, the authors recursively collected 
the related videos of every video in the list. They took the first step in studying popularity metrics other than viewcount,
but it was limited to four other variables only, \#comments, \#favorites, \#ratings, and the average rating.
They showed that all metrics, except the average rating, are highly correlated with the video viewcount
and that the correlation increases with video popularity.
They used linear regression to develop a model that evaluates the video viewcount
as a function of the \#favorites and \#ratings. The model could be used to detect
artificial boosting of video popularity.  Chatzopoulou at al. report the small world 
network properties for the related video graph by focusing on a subgraph of only popular nodes.

Our work is complementary to both previous works and more   
comprehensive, as we present analysis that allows us to understand which 
factors, among all possible video dependent or external factors,
are sources of influence on popularity. (What specifically
do we show regarding the referrers? - even for clones, same conclusion holds.
Also statistically show that search mechanisms are biased towards popular content
irrespective of the content.)

\subsubsection{Classification}

%Another issue is the focus on only classification~\cite{CrSo:08} or 
%   prediction~\cite{Huberman:10} while ignoring the temporal characteristics of popularity
%    evolution.

Other recent work on online popularity falls into clustering and 
classification systems. Crane and Sornette~\cite{CrSo:08} developed a 
method for classifying collective dynamics of a social system based on
whether the factor responsible for a viewing activity was caused by internal 
or external influences. The authors implicitly define internal and
external events through video referrers, and consider external links, embeds,
search links, and internal links as indognous factors, and featured
links as exogenous factors.  
%% Internal: eg. user searches - external: eg. featured or for example breaking news.
Crane and Sornette applied their model to
a time-series of views to 5 million YouTube videos, and 
based on the diversity in video popularity growth patterns, they labelled videos
as \textit{viral}, \textit{quality}, and \textit{junk}.
Popularity classes based on the heterogenity in popularity growth behavior
were also proposed in ~\cite{Google:10}, and explained by 
the level of socialness of a video. Video socialness is defined 
by assigning the video referrers as social
(external links and embeds) or non-social (search and internal mechanisms).
Even though different explanations were used for categorization in ~\cite{CrSo:08} 
and ~\cite{Google:10}, similar growth patterns were found across classes. 

Figueiredo et al.~\cite{Figueiredo:11} characterized the videos
belonging to the different datasets they collected into the classes defined by
Crane and Sornette~\cite{CrSo:08}. Based on the videos' popularity evolution patterns,
they classify the most popular video lists 
into the \textit{quality} category, whereas the list of deleted videos, 
and the list of videos obtained via keyword searches into the \textit{viral} category.



\subsubsection{Modeling and Prediction} 
%For intro line, check Tube over time conclusion
Szabo and Huberman \cite{Huberman:10} show again that there is a strong correlation between the logarithmically 
transformed total views early in the lifetime and later in the lifetime of 
the video. The authors model future total view counts as the sum of the 
current total view count, plus a linear term, that defines the 
relationships between the logarithmically transformed total view counts 
accumulated over times, and a noise term, that captures the randomness in 
the data. The model was validated with Youtube and Digg datasets collected similarly to our methodology. The error margin produced by their approach is relatively large because the percentage error is based on the total views since upload. 
Raktiewicz et al.~\cite{RMF+:10} presented a model
that combines the classical ``rich-get-richer'' model~\cite{Barabasi:99} with random bursts of 
popularity shifts, with the goal of capturing influence of exogenous
 events on popularity of content. The authors validated their model
 using click through data for  Wikipedia and the Chilean Web. 
%** Sampling Techniques 
%DATA

%Prior work on user-generated video popularity characteristics
%has typically relied either on network traffic traces from a
%network gateway~\cite{Mahanti:07, Zink08}  or 
%meta-data sampled  from video sharing services~\cite{Moon:09, MAY+09, Figueiredo:11}.

%one of these
%prior works~\cite{Moon:09, MAY+09, Figueiredo:11} 
%consider the issue of sampling biases, and in fact, Figueiredo et al. 
%point that the popularity characteristics of the three datasets
%are different. Our work builds upon this body of work by 
%studying how biases are introduced owing to sampling techniques, 
%and develops a methodology for studying the popularity dynamics
%of user-generated videos. %

%-Me: Figueiredo:11 even the random dataset is not random, 
%because we proved this method is biased, and they make it more biased 
%by selecting only the 1st result in every keyword search entry list.%

%We also note that a majority of the studies on video-sharing
%services have relied on meta-data collected via 
%crawling~\cite{Moon:09, Cheng:07,HaKe:07,Halvey:07, MAY+09, 
%Huberman:10, LeeMS:10, CrSo:08}.
%Cheng et al.~\cite{Cheng:07}  indicated that the usual crawling techniques 
%results with datasets biased towards popular content. In this paper, we 
%demonstrated that biases are introduced when keyword-search techniques
%are used for sampling videos. We also showed that popularity evolution
%can be studied in unbiased manner by tracking a collection of
%newly uploaded videos. 

%In ~\cite{Google:10}, sampling biases
%are introduced by limiting the analysis on videos with a certain
%%popularity threshold.
